Topological Strings on Toric geometries in the presence of Lagrangian branes

We propose expressions for refined open topological string partition function on certain non-compact Calabi Yau 3-folds with topological branes wrapped on the special lagrangian submanifolds. The corresponding web diagrams are partially compact and a lagrangian brane is inserted on one of the external legs. Partial compactification introduces a mass deformation in the corresponding gauge theory. We propose conjectures that equate these open topological string partition functions with the generating function of equivaraint indices on certain quiver moduli spaces. To obtain these conjectures we use the identification of topological string partition functions with equivariant indices on the instanton moduli spaces.

==> bibliography.tex <==
@article{Aganagic:2003db,
    author = "Aganagic, Mina and Klemm, Albrecht and Marino, Marcos and Vafa, Cumrun",
    title = "{The Topological vertex}",
    eprint = "hep-th/0305132",
    archivePrefix = "arXiv",
    reportNumber = "CALT-68-2439, HUTP-03-A032, HU-EP-03-24, CERN-TH-2003-111",
    doi = "10.1007/s00220-004-1162-z",
    journal = "Commun. Math. Phys.",
    volume = "254",
    pages = "425--478",
    year = "2005"
}
@article{Chuang:2013wpa,
    author = "Chuang, Wu-yen and Diaconescu, Duiliu-Emanuel and Donagi, Ron and Pantev, Tony",
    title = "{Parabolic refined invariants and Macdonald polynomials}",
    eprint = "1311.3624",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/s00220-014-2184-9",
    journal = "Commun. Math. Phys.",
    volume = "335",
    number = "3",
    pages = "1323--1379",
    year = "2015"
}
@book{MacDonald:2019755,
      author        = "MacDonald, Ian Grant and Zelevinsky, A V",
      title         = "{Symmetric functions and Hall polynomials; 2nd ed.}",
      publisher     = "Oxford University Press",
      address       = "Oxford",
      series        = "Oxford classic texts in the physical sciences",
      year          = "1998",
      url           = "https://cds.cern.ch/record/2019755",
}
@article{Chuang:2012dv,
    author = "Chuang, W.Y. and Diaconescu, D.E. and Pan, G.",
    editor = "Brambila-Paz, Leticia and Newstead, Peter and Thomas, Richard P. and Garc\'\i{}a-Prada, Oscar",
    title = "{BPS states and the P=W conjecture}",
    eprint = "1202.2039",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1017/CBO9781107279544.003",
    journal = "Lond. Math. Soc. Lect. Note Ser.",
    volume = "411",
    pages = "132--150",
    year = "2014"
}
@article{Chuang:2010ii,
    author = "Chuang, Wu-yen and Diaconescu, Duiliu-Emanuel and Pan, Guang",
    title = "{Wallcrossing and Cohomology of The Moduli Space of Hitchin Pairs}",
    eprint = "1004.4195",
    archivePrefix = "arXiv",
    primaryClass = "math.AG",
    reportNumber = "RUNHETC-2010-13",
    doi = "10.4310/CNTP.2011.v5.n1.a1",
    journal = "Commun. Num. Theor. Phys.",
    volume = "5",
    pages = "1--56",
    year = "2011"
}
@article{Bruzzo:2010fk,
    author = "Bruzzo, U. and Chuang, W.-y. and Diaconescu, D.-E. and Jardim, M. and Pan, G. and Zhang, Y.",
    title = "{D-branes, surface operators, and ADHM quiver representations}",
    eprint = "1012.1826",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "RUNHETC-2010-22",
    doi = "10.4310/ATMP.2011.v15.n3.a6",
    journal = "Adv. Theor. Math. Phys.",
    volume = "15",
    number = "3",
    pages = "849--911",
    year = "2011"
}
@article{Kozcaz:2018ndf,
    author = "Koz\c{c}az, Can and Shakirov, Shamil and Vafa, Cumrun and Yan, Wenbin",
    title = "{Refined Topological Branes}",
    eprint = "1805.00993",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "5",
    year = "2018"
}
@article{Jafarzade:2017fsc,
    author = "Jafarzade, Shahriyar and Nazari, Zainab",
    title = "{A New Integrable Ising-type Model from 2d $\mathcal{N}$=(2,2) Dualities}",
    eprint = "1709.00070",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "8",
    year = "2017"
}
@article{Deger:2018kur,
    author = "Deger, N.S. and Nazari, Z. and Sarioglu, O.",
    title = "{Supersymmetric solutions of N=(1,1) general massive supergravity}",
    eprint = "1803.06926",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.97.106022",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "10",
    pages = "106022",
    year = "2018"
}
@article{Kozcaz:2018ndf,
    author = "Koz\c{c}az, Can and Shakirov, Shamil and Vafa, Cumrun and Yan, Wenbin",
    title = "{Refined Topological Branes}",
    eprint = "1805.00993",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "5",
    year = "2018"
}
@article{Chuang:2013wpa,
    author = "Chuang, Wu-yen and Diaconescu, Duiliu-Emanuel and Donagi, Ron and Pantev, Tony",
    title = "{Parabolic refined invariants and Macdonald polynomials}",
    eprint = "1311.3624",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/s00220-014-2184-9",
    journal = "Commun. Math. Phys.",
    volume = "335",
    number = "3",
    pages = "1323--1379",
    year = "2015"
}
@article{Bastian:2018fba,
    author = "Bastian, Brice and Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Five-Dimensional Gauge Theories from Shifted Web Diagrams}",
    eprint = "1810.05109",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.99.046012",
    journal = "Phys. Rev. D",
    volume = "99",
    number = "4",
    pages = "046012",
    year = "2019"
}
@article{Sugimoto:2015nha,
    author = "Sugimoto, Yuji",
    title = "{The Enhancement of Supersymmetry in M-strings}",
    eprint = "1508.02125",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "OU-HET-867",
    doi = "10.1142/S0217751X16500883",
    journal = "Int. J. Mod. Phys. A",
    volume = "31",
    number = "16",
    pages = "1650088",
    year = "2016"
}
@misc{haiman2000hilbert,
    title={Hilbert schemes, polygraphs, and the Macdonald positivity conjecture},
    author={Mark Haiman},
    year={2000},
    eprint={math/0010246},
    archivePrefix={arXiv},
    primaryClass={math.AG}
}
@article{Chuang:2010ii,
    author = "Chuang, Wu-yen and Diaconescu, Duiliu-Emanuel and Pan, Guang",
    title = "{Wallcrossing and Cohomology of The Moduli Space of Hitchin Pairs}",
    eprint = "1004.4195",
    archivePrefix = "arXiv",
    primaryClass = "math.AG",
    reportNumber = "RUNHETC-2010-13",
    doi = "10.4310/CNTP.2011.v5.n1.a1",
    journal = "Commun. Num. Theor. Phys.",
    volume = "5",
    pages = "1--56",
    year = "2011"
}
@article{Haglund_2004,
   title={A combinatorial model for the Macdonald polynomials},
   volume={101},
   ISSN={1091-6490},
   url={http://dx.doi.org/10.1073/pnas.0405567101},
   DOI={10.1073/pnas.0405567101},
   number={46},
   journal={Proceedings of the National Academy of Sciences},
   publisher={Proceedings of the National Academy of Sciences},
   author={Haglund, J.},
   year={2004},
   month={Nov},
   pages={16127?16131}
}
@article{Iqbal:2015dra,
    author = "Iqbal, Amer and Khan, Ahsan Z. and Qureshi, Babar A. and Shabbir, Khurram and Shehper, Muhammad A.",
    title = "{Topological field theory amplitudes for A$_{N\ensuremath{-}1}$ fibration}",
    eprint = "1507.02662",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP12(2015)017",
    journal = "JHEP",
    volume = "12",
    pages = "017",
    year = "2015"
}
@article{Chuang:2012dv,
    author = "Chuang, W.Y. and Diaconescu, D.E. and Pan, G.",
    editor = "Brambila-Paz, Leticia and Newstead, Peter and Thomas, Richard P. and Garc\'\i{}a-Prada, Oscar",
    title = "{BPS states and the P=W conjecture}",
    eprint = "1202.2039",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1017/CBO9781107279544.003",
    journal = "Lond. Math. Soc. Lect. Note Ser.",
    volume = "411",
    pages = "132--150",
    year = "2014"
}
@inproceedings{MacDonald1998SymmetricFA,
  title={Symmetric functions and Hall polynomials},
  author={I. MacDonald},
  year={1998}
}
@article{Bruzzo:2010fk,
    author = "Bruzzo, U. and Chuang, W.-y. and Diaconescu, D.-E. and Jardim, M. and Pan, G. and Zhang, Y.",
    title = "{D-branes, surface operators, and ADHM quiver representations}",
    eprint = "1012.1826",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "RUNHETC-2010-22",
    doi = "10.4310/ATMP.2011.v15.n3.a6",
    journal = "Adv. Theor. Math. Phys.",
    volume = "15",
    number = "3",
    pages = "849--911",
    year = "2011"
}
@article{Iqbal:2009ki,
    author = "Iqbal, Amer and Kozcaz, Can and Sohail, Tanweer",
    title = "{Periodic Schur Process, Cylindric Partitions and N=2* Theory}",
    eprint = "0903.0961",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "3",
    year = "2009"
}
@article{Iqbal:2004ne,
    author = "Iqbal, Amer and Kashani-Poor, Amir-Kian",
    title = "{The Vertex on a strip}",
    eprint = "hep-th/0410174",
    archivePrefix = "arXiv",
    reportNumber = "SMS-0402, SLAC-PUB-10804, SU-ITP-04-39",
    doi = "10.4310/ATMP.2006.v10.n3.a2",
    journal = "Adv. Theor. Math. Phys.",
    volume = "10",
    number = "3",
    pages = "317--343",
    year = "2006"
}
@article{Taki:2008hb,
    author = "Taki, Masato",
    title = "{Flop Invariance of Refined Topological Vertex and Link Homologies}",
    eprint = "0805.0336",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "UT-08-14",
    month = "5",
    year = "2008"
}
@article{Iqbal:2012xm,
    author = "Iqbal, Amer and Vafa, Cumrun",
    title = "{BPS Degeneracies and Superconformal Index in Diverse Dimensions}",
    eprint = "1210.3605",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.90.105031",
    journal = "Phys. Rev. D",
    volume = "90",
    number = "10",
    pages = "105031",
    year = "2014"
}
@article{Iqbal:2007ii,
    author = "Iqbal, Amer and Kozcaz, Can and Vafa, Cumrun",
    title = "{The Refined topological vertex}",
    eprint = "hep-th/0701156",
    archivePrefix = "arXiv",
    doi = "10.1088/1126-6708/2009/10/069",
    journal = "JHEP",
    volume = "10",
    pages = "069",
    year = "2009"
}
@article{Iqbal:2012mt,
    author = "Iqbal, Amer and Kozcaz, Can",
    title = "{Refined topological strings on local $ {\mathrm{\mathbb{P}}}^2 $}",
    eprint = "1210.3016",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-PH-TH-2012-244",
    doi = "10.1007/JHEP03(2017)069",
    journal = "JHEP",
    volume = "03",
    pages = "069",
    year = "2017"
}
@article{Aganagic:2000gs,
    author = "Aganagic, Mina and Vafa, Cumrun",
    title = "{Mirror symmetry, D-branes and counting holomorphic discs}",
    eprint = "hep-th/0012041",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-00-A047",
    month = "12",
    year = "2000"
}
@article{Aganagic:2001nx,
    author = "Aganagic, Mina and Klemm, Albrecht and Vafa, Cumrun",
    title = "{Disk instantons, mirror symmetry and the duality web}",
    eprint = "hep-th/0105045",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-01-A023, HU-EP-01-21",
    doi = "10.1515/zna-2002-1-201",
    journal = "Z. Naturforsch. A",
    volume = "57",
    pages = "1--28",
    year = "2002"
}
@article{Neitzke:2004ni,
    author = "Neitzke, Andrew and Vafa, Cumrun",
    title = "{Topological strings and their physical applications}",
    eprint = "hep-th/0410178",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-04-A039",
    month = "10",
    year = "2004"
}
@article{Hollowood:2003cv,
    author = "Hollowood, Timothy J. and Iqbal, Amer and Vafa, Cumrun",
    title = "{Matrix models, geometric engineering and elliptic genera}",
    eprint = "hep-th/0310272",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-03-A074",
    doi = "10.1088/1126-6708/2008/03/069",
    journal = "JHEP",
    volume = "03",
    pages = "069",
    year = "2008"
}

@article{Hollowood:2003gr,
    author = "Hollowood, Timothy J.",
    title = "{Five-dimensional gauge theories and quantum mechanical matrix models}",
    eprint = "hep-th/0302165",
    archivePrefix = "arXiv",
    doi = "10.1088/1126-6708/2003/03/039",
    journal = "JHEP",
    volume = "03",
    pages = "039",
    year = "2003"
}
@article{Hohenegger:2013ala,
    author = "Hohenegger, Stefan and Iqbal, Amer",
    title = "{M-strings, elliptic genera and $\mathcal{N} = 4$ string amplitudes}",
    eprint = "1310.1325",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-PH-TH-2013-237",
    doi = "10.1002/prop.201300035",
    journal = "Fortsch. Phys.",
    volume = "62",
    pages = "155--206",
    year = "2014"
}
@inproceedings{Gritsenko:1999nm,
    author = "Gritsenko, V.",
    title = "{Complex vector bundles and Jacobi forms}",
    eprint = "math/9906191",
    archivePrefix = "arXiv",
    month = "1",
    year = "1999"
}
@article{Haghighat:2013gba,
    author = "Haghighat, Babak and Iqbal, Amer and Koz\c{c}az, Can and Lockhart, Guglielmo and Vafa, Cumrun",
    title = "{M-Strings}",
    eprint = "1305.6322",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/s00220-014-2139-1",
    journal = "Commun. Math. Phys.",
    volume = "334",
    number = "2",
    pages = "779--842",
    year = "2015"
}
@article{Li:2004ef,
    author = "Li, Jun and Liu, Kefeng and Zhou, Jian",
    title = "{Topological string partition functions as equivariant indices}",
    eprint = "math/0412089",
    archivePrefix = "arXiv",
    month = "12",
    year = "2004"
}
@article{Antoniadis:1993ze,
    author = "Antoniadis, Ignatios and Gava, E. and Narain, K.S. and Taylor, T.R.",
    title = "{Topological amplitudes in string theory}",
    eprint = "hep-th/9307158",
    archivePrefix = "arXiv",
    reportNumber = "NUB-3071, IC-93-202, CPTH-A258-0793",
    doi = "10.1016/0550-3213(94)90617-3",
    journal = "Nucl. Phys. B",
    volume = "413",
    pages = "162--184",
    year = "1994"
}
@article{Aharony:1997bh,
    author = "Aharony, Ofer and Hanany, Amihay and Kol, Barak",
    title = "{Webs of (p,q) five-branes, five-dimensional field theories and grid diagrams}",
    eprint = "hep-th/9710116",
    archivePrefix = "arXiv",
    reportNumber = "IASSNS-HEP-97-113, RU-97-81, SU-ITP-97-40",
    doi = "10.1088/1126-6708/1998/01/002",
    journal = "JHEP",
    volume = "01",
    pages = "002",
    year = "1998"
}
@article{Leung:1997tw,
    author = "Leung, Naichung Conan and Vafa, Cumrun",
    title = "{Branes and toric geometry}",
    eprint = "hep-th/9711013",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-97-A090",
    doi = "10.4310/ATMP.1998.v2.n1.a4",
    journal = "Adv. Theor. Math. Phys.",
    volume = "2",
    pages = "91--118",
    year = "1998"
}
@article{Iqbal:2008ra,
    author = "Iqbal, Amer and Kozcaz, Can and Shabbir, Khurram",
    title = "{Refined Topological Vertex, Cylindric Partitions and the U(1) Adjoint Theory}",
    eprint = "0803.2260",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1016/j.nuclphysb.2010.06.010",
    journal = "Nucl. Phys. B",
    volume = "838",
    pages = "422--457",
    year = "2010"
}
@article{Iqbal:2003zz,
    author = "Iqbal, Amer and Kashani-Poor, Amir-Kian",
    title = "{SU(N) geometries and topological string amplitudes}",
    eprint = "hep-th/0306032",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-9924, HUTP-03-A038, SU-ITP-03-12",
    doi = "10.4310/ATMP.2006.v10.n1.a1",
    journal = "Adv. Theor. Math. Phys.",
    volume = "10",
    number = "1",
    pages = "1--32",
    year = "2006"
}
@article{Iqbal:2003ix,
    author = "Iqbal, Amer and Kashani-Poor, Amir-Kian",
    title = "{Instanton counting and Chern-Simons theory}",
    eprint = "hep-th/0212279",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-9623, HUTP-02-A064, SU-ITP-02-48",
    doi = "10.4310/ATMP.2003.v7.n3.a4",
    journal = "Adv. Theor. Math. Phys.",
    volume = "7",
    number = "3",
    pages = "457--497",
    year = "2003"
}
@article{Bonelli:2019het,
    author = "Bonelli, Giulio and Fasola, Nadir and Tanzini, Alessandro",
    title = "{Flags of sheaves, quivers and symmetric polynomials}",
    eprint = "1911.12787",
    archivePrefix = "arXiv",
    primaryClass = "math.AG",
    month = "11",
    year = "2019"
}
@phdthesis{Assi:2014exa,
    author = "Zein Assi, Ahmad",
    title = "{Topological Amplitudes and the String Effective Action}",
    eprint = "1402.2428",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "TEL-00942993",
    school = "Ecole Polytechnique, CPHT",
    year = "2013"
}
@article{Fantechi_2010,
   title={Riemann?Roch theorems and elliptic genus for virtually smooth schemes},
   volume={14},
   ISSN={1465-3060},
   url={http://dx.doi.org/10.2140/gt.2010.14.83},
   DOI={10.2140/gt.2010.14.83},
   number={1},
   journal={Geometry and Topology},
   publisher={Mathematical Sciences Publishers},
   author={Fantechi, Barbara and Gottsche, Lothar},
   year={2010},
   month={Jan},
   pages={83?115}
}
@article{AIqbalsms,
    author = "Amer Iqbal ",
    title = "{Unpublished notes}",
%    eprint = "1911.12787",
%    archivePrefix = "arXiv",
%    primaryClass = "math.AG",
%    month = "11",
%    year = "2019"
}

